Overcoming Oversmoothness in Graph Convolutional Networks via Hybrid Scattering Networks

Geometric deep learning has made great strides towards generalizing the design of structure-aware neural networks from traditional domains to non-Euclidean ones, giving rise to graph neural networks (GNN) that can be applied to graph-structured data arising in, e.g., social networks, biochemistry, and material science. Graph convolutional networks (GCNs) in particular, inspired by their Euclidean counterparts, have been successful in processing graph data by extracting structure-aware features. However, current GNN models are often constrained by various phenomena that limit their expressive power and ability to generalize to more complex graph datasets. Most models essentially rely on low-pass filtering of graph signals via local averaging operations, leading to oversmoothing. Moreover, to avoid severe oversmoothing, most popular GCN-style networks tend to be shallow, with narrow receptive fields, leading to underreaching. Here, we propose a hybrid GNN framework that combines traditional GCN filters with band-pass filters defined via geometric scattering. We further introduce an attention framework that allows the model to locally attend over combined information from different filters at the node level. Our theoretical results establish the complementary benefits of the scattering filters to leverage structural information from the graph, while our experiments show the benefits of our method on various learning tasks.

==> Tables/alpha_accuracy.tex <==
\begin{table}[h]
\small
\begin{minipage}{0.9\textwidth}
%% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption*{Classification accuracies on ogbn-proteins dataset with different $\alpha$. }\label{tab:alpha_parameter}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$\alpha$  & 0.1 & 0.5 & 1.0 & 3. & 5.0 \\\hline
Classification Accuracy  & $72.03 \pm 0.81$ & $72.45 \pm 1.30$ & $73.93 \pm 0.19$ & $72.23 \pm 0.45$  & $71.45 \pm 1.41$ \\ \hline
\end{tabular}
\end{minipage}
\end{table}

==> Tables/smoothness.tex <==
\begin{table}[h]
%% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{Comparison of GCN's performance with number of layers on DBLP dataset (higher is better).}\label{tab:smoothness}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Number of layers   & 2 & 4 & 8 & 16 \\\hline
Smoothness on top-$1$  & 0.2018 & 0.2756 & 0.1969 & 0.082\\ \hline
Percentage of top-$1$   & 55.23\% &48.59\% & 47.21\% & 96.82\%\\ \hline
Classification accuracy  & 72.05\%& 40.00\% & 4.10\% & 5.60\%\\ \hline
\end{tabular}
\end{table}
\textcolor{blue}{add sct smoothness}

==> journal-rewrite/frame_properties.tex <==
{\color{blue}
\subsection{Energy Preservation}\label{sec:apx-frame}

Let us consider the a weighted inner product space $\bL^2(\bM)$ of signals supported on $V$ with inner product $\langle \bx, \by \rangle_{\bM} \coloneqq \langle \bM\bx, \bM\by \rangle_2$, where $\langle\cdot,\cdot \rangle_2$ denotes the standard inner product on $\R^n$. We further write $\bu_i \coloneqq \bD^{1/2}\bq_i$. 

\textcolor{red}{Its probably worht noting $<x,y>_{D^{-1/2}}$ has the nice form $\sum_{i=1}^N \frac{x_iy_i}{d_i}$ or more generally if we pick $M=D^{\alpha}$ we have $<x,y>=\sum_{i=1}^Nx_iy_id_i^{2\alpha}$}

\begin{defn}\label{def:frame}
    A set of matrices $\mathcal{W} = \{\bB_k\}_{k\in\mathcal{I}}$ is called \textit{frame} if there exist constants $0 < c < C < \infty$ such that
    $ %$\begin{equation}\label{eq:frame}
        c \Vert\bx\Vert_{\bM}^2 \leq \Vert\mathcal{W}_K\Vert_{\bM}^2 \coloneqq \sum_{k=0}^K \Vert\bB\Vert_{\bM}^2 \leq C \Vert\bx\Vert_{\bM}^2.
    $ %\end{equation}
    If additionally $C=1$, we speak of a \textit{non-expansive frame}.
\end{defn}

\begin{prop}[\cite{perlmutter2019understanding}]\label{prop:frame}
    For $\bM = \bD^{-1/2}$, the filter bank $\mathcal{W}_1 \coloneqq \{\boldsymbol{\Psi}_k, \boldsymbol{\Phi}_K\}_{k=0}^K$ is a non-expansive frame with universal constants $c_1>0$ and $C_1=1$.
\end{prop}

The low-pass filters in our model are based on GCN filters. Although conceptually filling the same role, they do not satisfy the assumptions of Prop.~\ref{prop:frame}. However, we can show a similar result when disregarding the low-pass filters.

\begin{prop}\label{prop:frame-band}
    For $\bM = \bD^{-1/2}$ and signals $\bx\in\R^n$ with $\langle \bx, \bu_1 \rangle_{\bM} = 0$, the filter bank $\mathcal{W}_2 \coloneqq \{\boldsymbol{\Psi}_k\}_{k=0}^K$ is a non-expansive frame with $c_2=c_2(\lambda_2)$ depending on the Fiedler value (and hence the graph structure) and $C_2=1$.
\end{prop}

The assumption $\bx \perp \bv_1$ is necessary to retrieve a non-trivial lower bound $c_2>0$ as $\bPsi_k \bu_1 = 0$ for all $k\geq 0$.

\begin{proof}
    Let us define $P_{\mathcal{W}}(t)\coloneqq \sum_{\bB\in \mathcal{W}} p_{\bB}(t)^2$. We can use the result from the proof of Prop.~2.2 in~\cite{perlmutter2019understanding} that the lower frame bound of $\mathcal{W}_2$ can be deduced from $\min_{2\leq i\leq n} P_{\mathcal{W}_2}$. Note that $i=1$ is not considered as we assumed $\bx \perp \bu_1$. This gives
    $
        \min_{2\leq i\leq n} P_{\mathcal{W}_2}(\lambda_i) \geq \min_{2\leq i\leq n} p_{\bPsi_0}(\lambda_i) \geq (1 - \omega_2)^2 \eqqcolon c_2.
    $
    The upper frame bound is easily derived from Prop.~\ref{prop:frame} as $\Vert \boldsymbol{\Phi}_K\Vert_{\bM}^2 \geq 0$.
\end{proof}

For context, let us investigate another filter bank that only uses low-pass filters $\mathcal{W}_3 \coloneqq \{\bPhi_k\}_{k=0}^K$. Notably, the filters in $\mathcal{W}_3$ have receptive fields of size equal to the filters in $\mathcal{W}_2$. However, $\mathcal{W}_3$ exhibits considerably weaker energy preservation properties.
\textcolor{red}{For GCN style filters, the unweighted space is more natural since they are symmetric matrices}
\begin{prop}\label{prop:frame-low}
    For $\bM = \bD^{-1/2}$, $\mathcal{W}_3$ is a frame with $c_3 = c_3(\lambda_n)$ and $C_3 = C_3(\lambda_1)$. Further, $\mathcal{W}_3$ has the following properties:
    \begin{enumerate}
        \item[(a)] $\mathcal{W}_3$ is not non-expansive.
        \item[(b)] It holds $C_3 > 1 = C_2 = C_1$.
        \item[(c)] It holds $0 < c_3 < c_2$.
    \end{enumerate}
\end{prop}

\begin{proof}
    Let us start by showing that $\mathcal{W}_3$ is a non-expansive frame. For the lower frame bound, we have that $\min_{2\leq i\leq n} P_{\mathcal{W}_3}(\omega_i) \geq \min_{1\leq i\leq n} p_{\bPhi_0}(\omega_i)^2 \geq \omega_n^2 \eqqcolon c_3$. For the upper frame bound, we use the geometric series to bound $P_{\mathcal{W}_3}$ from above via
    $
        P_{\mathcal{W}_3}(\omega_i) = \sum_{k=0}^K \big(\omega_i^{2^k}\big)^2 < \sum_{k=0}^{2^{K+1}} \omega_i^k = (1 - \omega_i^{2^{K+1} + 1}) / (1 - \omega_i).
    $
    Therefore, we have $C_3 \coloneqq \sup_{\omega\in (0,1]} (1 - \omega^{2^{K+1} + 1}) / (1 - \omega) > 1.$
    {\color{brown}
    The function $g(\omega) \coloneqq (1 - \omega^{2^{K+1} + 1}) / (1 - \omega)$ is continuous and increases monotonously on $[0,1)$. It can be continuously extended to $t=1$ and, in particular, attains its maximum at the same point, i.e., $C_3 = \lim_{\omega\nearrow 1} g(\omega) = 2^{K+1} + 1$ using L'Hôpital's rule.}
    This in turn establishes claim (a) and (b).
\end{proof}

}
